Smart pixel sensors: towards on-sensor filtering of pixel clusters with deep learning

Highly granular pixel detectors allow for increasingly precise measurements of charged particle tracks. Next-generation detectors require that pixel sizes will be further reduced, leading to unprecedented data rates exceeding those foreseen at the High Luminosity Large Hadron Collider. Signal processing that handles data incoming at a rate of O(40MHz) and intelligently reduces the data within the pixelated region of the detector at rate will enhance physics performance at high luminosity and enable physics analyses that are not currently possible. Using the shape of charge clusters deposited in an array of small pixels, the physical properties of the traversing particle can be extracted with locally customized neural networks. In this first demonstration, we present a neural network that can be embedded into the on-sensor readout and filter out hits from low momentum tracks, reducing the detector's data volume by 54.4-75.4%. The network is designed and simulated as a custom readout integrated circuit with 28 nm CMOS technology and is expected to operate at less than 300 $\mu W$ with an area of less than 0.2 mm$^2$. The temporal development of charge clusters is investigated to demonstrate possible future performance gains, and there is also a discussion of future algorithmic and technological improvements that could enhance efficiency, data reduction, and power per area.

==> sections/2-dataset/dataReductionWithUntracked.tex <==
\begin{table}[!htp]
\begin{center}
\begin{tabular}{llll}
\textbf{Model} & \textbf{Test Set} & \textbf{W/ untracked clusters} & \textbf{W/ untracked clusters $\&$ single pixel hits}\\\hline
Model 1 &  \% &  \%  &  \% \\

\hline
\end{tabular}
\caption{new data reduction numbers}
\label{reduction}
\end{center}
\end{table}

==> sections/2-dataset/dataset-v1.tex <==
\section{Geometry and Dataset (Jennet, Morris)}
\label{sec:dataset}

This study is based on a simulated dataset of silicon pixel clusters produced by charged particles (pions), where the particle kinematics are taken from fitted tracks in CMS Run 2 data \cite{zenodo}. 
 %{Comment about non-tracked clusters aren't apart of this study (AB)} 
 The interaction of the charged particles with a 100\,$\mu m$ thick silicon pixel detector is simulated using a time-sliced version of PixelAV \cite{pixelav}. The pixel detector is taken to be a 21x13 array of pixels with 50x12.5 micron pitch, situated 30mm from the particle's origin point (see Figure \ref{pTcartoon}). The detector is immersed in a 3.8T magnetic field parallel to the sensor x coordinate. 

The position $(x,y)$ where the charged particle traverses the sensor mid-plane is uniformly distributed across the central 3x3 pixel array. The shape of the charge deposited in the pixel array is sensitive to this position and to the particle's angle of incidence. The track angle in the $x-z$ plane is denoted by $\alpha$, and by $\beta$ in the $y-z$ plane. Due to bending in the plane of the magnetic field, the shape of the charge cluster also depends on the particle's transverse momentum ($p_T$), which is highly correlated with $\beta$.  The shape of the cluster also depends strongly on its azimuthal position with respect to the center of the sensor, which is denoted by the coordinate $y$ in Figure \ref{pTcartoon}. 

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.45\textwidth]{sections/2-dataset/figures/sensor-smart-pixel.pdf}
  \hspace{0.5cm}
  \includegraphics[width=0.4\textwidth]{sections/2-dataset/figures/pTcartoon.pdf}
   \caption{A diagram of three charged particle tracks traversing our simulated silicon sensor at the same $y$ position. The sensor is viewed in the bending plane of the magnetic field. The solid track corresponds to a charged particle track with high $p_T$, while the two dashed tracks correspond to low $p_T$ tracks from particles with opposite charge. \nvt{Can we add a second figure (left) that shows the whole sensor imagined?}}
  \label{pTcartoon}
\end{figure}

The distribution of particle $p_T$ is shown in Figure \ref{pT}. The number of particles increases with decreasing $p_T$, but few particles with very low $p_T$ are reconstructed as tracks in CMS. As a result, the track $p_T$ distribution begins around 200 MeV. The signatures of lower $p_T$ particles are dominated by single pixel hits. 

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.6\textwidth]{sections/2-dataset/figures/pT.pdf}
   \caption{Transverse momentum ($p_T$) of simulated tracks in the dataset.}
  \label{pT}
\end{figure}

For a given cluster, the sum over pixel columns projects the cluster shape onto the $x$-axis: this distribution is referred to as the \textbf{x-profile}. The sum over pixel rows, \textbf{y-profile}, which projects the cluster shape onto the y-axis, is sensitive to incident angle $\beta$ and therefore to the track $p_T$.  The mean y-profile charge distributions for tracks impinging near the center of a sensor ($-1 < y_0 < 1$) shown in Figure \ref{yprofile} for three populations of clusters. Clusters created by high $p_T$ particles ($p_T > 2$ GeV) are represented by the black distribution, while clusters created by low $p_T$ particles ($p_T < 200$ MeV) are represented by red and blue for positively and negatively charged particles, respectively. 

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.4\textwidth]{sections/2-dataset/figures/yprofile_9.pdf}
   \caption{Distribution of y-profile cluster size for positively charged low $p_T$ particles (red), negatively charged low $p_T$ particles (blue) and high $p_T$ particles of both signs (black). Each distribution includes tracks that are approximately normal to the sensor ($-1 < y_0 < 1$). }
  \label{yprofile}
\end{figure}

Due to the deflection of charge carriers by the magnetic field (Lorentz drift), the cluster shape is not symmetric in $\beta$. For a flat detector module that measures 16 mm in y, particles of similar momentum leave markedly different cluster shapes at different positions $y_0$ on the module. Figure \ref{yprofile2} shows the average cluster shapes at the extreme edges of the module, and can be compared with Figure \ref{yprofile}. 

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.4\textwidth]{sections/2-dataset/figures/yprofile_0.pdf}
  \includegraphics[width=0.4\textwidth]{sections/2-dataset/figures/yprofile_7.pdf}
   \caption{Distribution of y-profile at extreme $y_0$: (left) $-8 < y_0 < -6$ mm and (right) $6 < y_0 < 8$ mm. Shown separately for positively charged low $p_T$ particles (red), negatively charged low $p_T$ particles (blue) and high $p_T$ particles of both signs (black). Taken with Figure \ref{yprofile}, the cluster shape dependence on $y_0$ is clear.}
  \label{yprofile2}
\end{figure}

The cluster $y$ size is defined as the number of pixel rows in which non-zero net charge has been deposited after 4 ns. The dependence of the cluster $y$ size on both the charged particle $p_T$ and $y_0$ is shown in Figure \ref{sizeVsYlocal}. The decrease in y size from the left to right edge of the flat module is due to Lorentz drift. 

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.7\textwidth]{sections/2-dataset/figures/ylocal_ysize.pdf}
   \caption{Cluster $y$ size vs $y_0$ for different values of particle charge and $p_T$. The decrease in cluster size from the left to right side of the sensor plane is due to Lorentz drift.}
  \label{sizeVsYlocal}
\end{figure}

In order to study the potential gain from timing information, the simulation also records the induced and collected charge in each pixel at 200 picosecond time intervals. The evolution of an example cluster is shown in Figure \ref{timing}.

\begin{figure}[htbp]
  \centering
  \subfloat[$t=0$]{\includegraphics[width=0.45\textwidth]{sections/2-dataset/figures/slices_ev02_sl00.png}}
  \subfloat[$t=200$ps]{\includegraphics[width=0.45\textwidth]{sections/2-dataset/figures/slices_ev02_sl01.png}}\\
  \subfloat[$t=400$ps]{\includegraphics[width=0.45\textwidth]{sections/2-dataset/figures/slices_ev02_sl02.png}}
  \subfloat[$t=600$ps]{\includegraphics[width=0.45\textwidth]{sections/2-dataset/figures/slices_ev02_sl03.png}}\\
  \subfloat[$t=1800$ps]{\includegraphics[width=0.45\textwidth]{sections/2-dataset/figures/slices_ev02_sl09.png}}
  \subfloat[$t=3000$ps]{\includegraphics[width=0.45\textwidth]{sections/2-dataset/figures/slices_ev02_sl15.png}}
   \caption{Time evolution of a charge cluster in the simulated 21x13 pixel array. The color scale represents the number of electrons collected after the time denoted.}
  \label{timing}
\end{figure}

\FloatBarrier


==> sections/3-task-and-algorithm/efficiency.tex <==
\begin{table}[!htp]
\begin{center}
\begin{tabular}{ll}
\textbf{Minimum $p_T$} & \textbf{Rejected tracks} \\ \hline
0.2 GeV & 6\%\\
0.5 GeV & 36\%\\
1 GeV & 70\%\\
2 GeV & 94\%\\
\hline
\end{tabular}
\caption{Fraction of tracks rejected by the application of a minimum $p_T$ cut to the dataset described in Section \ref{sec:dataset}.}
\label{eff-pt-cut}
\end{center}
\end{table}


==> sections/3-task-and-algorithm/noise-threshold.tex <==
\begin{table}[!htp]
\begin{center}
\begin{tabular}{lllll}
\textbf{Threshold [$e^-$]} & \textbf{0.2 GeV} & \textbf{0.5 GeV} & \textbf{1 GeV} & \textbf{2 GeV} \\ \hline
0 & 78.2 \% & 88.2 \% &  91.0 \% & 92.6 \%\\
400 & 77.5 \% & 85.6 \% &  87.5 \% & 88.3 \%\\
600 & 74.4 \% & 82.2 \% &  84.3 \% & 85.9 \%\\
800  & 75.3 \% & 82.2 \% &  84.3 \% & 86.0 \%\\
\hline
\end{tabular}
\caption{Model Performance: Accuracy of the baseline model using different thresholds\cm{What are the columns here? should be discussed in the text as well.}}
\label{noise-threshold}
\end{center}
\end{table}

==> sections/3-task-and-algorithm/quantized-accuracy.tex <==
\begin{table}[!htp]
\begin{center}
\begin{tabular}{lllll}
\textbf{Input} & \textbf{0.2 GeV} & \textbf{0.5 GeV} & \textbf{1 GeV} & \textbf{2 GeV} \\ \hline
Timeslices & 82.3 \% & 95.2 \% &  97.3 \% & 97.6 \%\\
Full Precision & 78.2 \% & 88.2 \% &  91.0 \% & 92.6 \%\\
Quantized Inputs & 76.8 \% & 85.2 \% &  87.8 \% & 88.6 \%\\
QKeras & 77.5 \% & 85.6 \% &  87.5 \% & 88.3 \%\\
YSize & 73.1 \% & 79.0 \% &  81.0 \% & 82.9 \%\\
\hline
\end{tabular}
\caption{Model Performance: Accuracy }
\end{center}
\label{quantized-accuracy}
\end{table}

==> sections/3-task-and-algorithm/quantized-tpr-fpr.tex <==
%False Positive - predict low, actually high - wrongly keep this high pT cluster
%False Negative - predict high, true low - wrongly reject
\begin{table}[!htp]
\begin{center}
\begin{tabular}{lll}
\textbf{Model} & \textbf{False Positive Rate} & \textbf{False Negative Rate} \\ \hline
Timeslices & 8.9 \% & 8.1 \%\\
Full Precision & 10.9 \% & 13.4 \%\\
Quantized Inputs & 11.6 \% & 15.2 \%\\
QKeras & 11.3 \% & 16.0 \%\\
YSize & 13.4 \% & 20.7 \%\\
\hline
\end{tabular}
\caption{Model Performance: True and False Positive Rates - percentages have denominator =  number of test clusters == 163040 - to do double check numbers with confusion matrix}
\end{center}
\end{table}

%\begin{table}[!htp]
%\begin{center}
%\begin{tabular}{lll}
%\textbf{Model} & \textbf{False Positive Rate} & \textbf{False Negative Rate} \\ \hline
%Timeslices & 17.7 \% & 16.2 \%\\
%Full Precision & 21.9 \% & 26.8 \%\\
%Quantized Inputs & 23.3 \% & 30.4 \%\\
%%QKeras & 22.5 \% & 32.0 \%\\
%YSize & 26.9 \% & 41.3 \%\\
%\hline
%\end{tabular}
%\caption{Model Performance: True and False Positive Rates  - percentages have denominator =  number of low or high pt clusters == 81520}
%\end{center}
%\end{table}

%https://docs.google.com/spreadsheets/d/1pzYggtgjU-Q__qwM8frH2nJFT5p6v-bnHO5MtJzeoic/edit?usp=sharing 

==> sections/3-task-and-algorithm/reduction-quantized.tex <==
%False Positive - predict low, actually high - wrongly keep this high pT cluster
%False Negative - predict high, true low - wrongly reject
\begin{table}[!htp]
\begin{center}
\begin{tabular}{llll}
\textbf{Model} & \textbf{Data Reduction} & \textbf{False Positives} & \textbf{False Negatives} \\ \hline
Full precision & 65.8 \% &  10.9\%  & 13.4 \% \\
Quantized inputs &  68.8 \% & 11.6 \% & 15.2 \%  \\
Quantized weights \& inputs & 70.8 \% &  11.3\%  &  16.0\% \\
\hline
\end{tabular}
\caption{Comparison of model performance in terms of data reduction, false positive rate, and false negative rate at different stages of the quantization.}
\label{reduction-quantized}
\end{center}
\end{table}

==> sections/3-task-and-algorithm/reduction.tex <==
\begin{table}[!htp]
\begin{center}
\begin{tabular}{llll}
\textbf{Model} & \textbf{Data Reduction} & \textbf{False Positives} & \textbf{False Negatives} \\ \hline
Model 1 &  77.9 \% &  13.4\% & 20.7 \% \\
Model 2 & 65.8 \% &  10.9\%  & 13.4 \% \\
Model 3 & 57.4 \% & 8.9 \%  &   8.1\% \\
\hline
\end{tabular}
\caption{Comparison of model performance in terms of data reduction, false positive rate, and false negative rate. \kdp{would be useful to include signal efficiency for tracks with $p_T > 2$~GeV}}
\label{reduction}
\end{center}
\end{table}

==> sections/9-modelExploration/training.tex <==
\section{Training}
\label{app:loss curves}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.30\textwidth]{sections/3-task-and-algorithm/figures/arch1.png}
  \hspace{0.5cm}
  \includegraphics[width=0.5\textwidth]{sections/3-task-and-algorithm/figures/archTS.png}
   \caption{Model architecture of Model 2 ($y$-profile) (left) and Model 3 ($y$-profile + time) (right). Each $3\times2$ table represents one layer in the network. The first column of each table shows the name and type of the layer, and the last column shows the shape of the input and output data (top and bottom respectively). }
  \label{arch-model2}
\end{figure}

\begin{figure}[htbp]
  \centering
  \subfloat[]{\includegraphics[width=0.48\textwidth]{sections/3-task-and-algorithm/figures/accuracy_fullPrecision.png}}
  \subfloat[]{\includegraphics[width=0.48\textwidth]{sections/3-task-and-algorithm/figures/loss_fullPrecision.png}}
   \caption{Training performance of Model 2: (a) evolution of the classifier accuracy with each training epoch, and (b) evolution of the loss with each training epoch.}
  \label{val-model2}
\end{figure}

\begin{figure}[htbp]
  \centering
  \subfloat[]{\includegraphics[width=0.48\textwidth]{sections/3-task-and-algorithm/figures/accuracy_TS.png}}
  \subfloat[]{\includegraphics[width=0.48\textwidth]{sections/3-task-and-algorithm/figures/loss_TS.png}}
   \caption{Training performance of Model 3: (a) evolution of the classifier accuracy with each training epoch, and (b) evolution of the loss with each training epoch.}
  \label{val-model3}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.48\textwidth]{sections/3-task-and-algorithm/figures/accuracy_QuantInputQuantYLocal64.png}
  \includegraphics[width=0.48\textwidth]{sections/3-task-and-algorithm/figures/loss_QuantInputQuantYLocal64.png}
   \caption{Training performance of the quantized Model 2: (a) evolution of the classifier accuracy with each training epoch, and (b) evolution of the loss with each training epoch.}
  \label{val-qmodel2}
\end{figure}






\begin{figure}
  \centering
  \includegraphics[width=0.65\textwidth]{sections/3-task-and-algorithm/figures/compareThresholds.png}
   \caption{Classifier acceptance vs. $p_T$ for the quantized Model 2, with each curve corresponding to a different value of the minimum noise threshold. Positive and negative values of $p_T$ represent the performance on clusters initiated by particles of positive and negative charge, respectively.}
  \label{thresholds}
\end{figure}

\FloatBarrier

